Open-Set Domain Adaptation for Semantic Segmentation

Unsupervised domain adaptation (UDA) for semantic segmentation aims to transfer the pixel-wise knowledge from the labeled source domain to the unlabeled target domain. However, current UDA methods typically assume a shared label space between source and target, limiting their applicability in real-world scenarios where novel categories may emerge in the target domain. In this paper, we introduce Open-Set Domain Adaptation for Semantic Segmentation (OSDA-SS) for the first time, where the target domain includes unknown classes. We identify two major problems in the OSDA-SS scenario as follows: 1) the existing UDA methods struggle to predict the exact boundary of the unknown classes, and 2) they fail to accurately predict the shape of the unknown classes. To address these issues, we propose Boundary and Unknown Shape-Aware open-set domain adaptation, coined BUS. Our BUS can accurately discern the boundaries between known and unknown classes in a contrastive manner using a novel dilation-erosion-based contrastive loss. In addition, we propose OpenReMix, a new domain mixing augmentation method that guides our model to effectively learn domain and size-invariant features for improving the shape detection of the known and unknown classes. Through extensive experiments, we demonstrate that our proposed BUS effectively detects unknown classes in the challenging OSDA-SS scenario compared to the previous methods by a large margin. The code is available at https://github.com/KHU-AGI/BUS.

==> ddd.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary

%\section{Appendix}
%\label{sec:rationale}
%\section{Rationale}
%\label{sec:rationale}
% 
%Having the supplementary compiled together with the main paper means that:
% 
%\begin{itemize}
%\item The supplementary can back-reference sections of the main paper, for example, we can refer to \cref{sec:intro};
%\item The main paper can forward reference sub-sections within the supplementary explicitly (e.g. referring to a particular experiment); 
%\item When submitted to arXiv, the supplementary will already be included at the end of the paper. ~\cite{berthelot2019mixmatch}
%\end{itemize}
% 
%To split the supplementary pages from the main paper, you can use \href{https://support.apple.com/en-ca/guide/preview/prvw11793/mac#:~:text=Delete%20a%20page%20from%20a,or%20choose%20Edit%20%3E%20Delete).}{Preview (on macOS)}, \href{https://www.adobe.com/acrobat/how-to/delete-pages-from-pdf.html#:~:text=Choose%20%E2%80%9CTools%E2%80%9D%20%3E%20%E2%80%9COrganize,or%20pages%20from%20the%20file.}{Adobe Acrobat} (on all OSs), as well as \href{https://superuser.com/questions/517986/is-it-possible-to-delete-some-pages-of-a-pdf-document}{command line tools}.

%\subsection{OpenReMix}
%\label{sec:OpenReMix}
%\paragraph{Resizing Object.}

%\documentclass{book}
%\usepackage[toc,title,page]{appendix}

%\begin{document}

%\tableofcontents

\appendix
%\renewcommand{\thesection}{\Alph{section}.\arabic{section}}
\setcounter{section}{0}
\setcounter{figure}{0}
\setcounter{table}{0}


\begin{appendix}
%\section{Overview}
%Some text
\section{More Details of BUS}
In this section, we provided further implementation details of the proposed method. 

In the DECON loss, the dilation and erosion functions vary in the extent of dilation and erosion depending on the kernel size and number of iterations. In this study, we utilized a 3$\times$3 kernel size and 1 iteration. Moreover, we used random crop size as 64$\times$64 for the target private map. For OpenReMix, we used the resized source image $x_s^r$, utilizing bilinearly downsampling $\zeta(\cdot,\cdot)$ on source image $x_s$ with scale factor $s_r$, \textit{e.g.}, $x_s^r= \zeta(x_s,s_r)$. The $s_r$ determines the extent of resizing for the thing class from the source image. As shown in Figure~\ref{fig:OpenReMix}, we set the scale factor $s_r$ to 0.5 and we represented the resized thing class as a yellow mask.

% An example of the resized thing class is shown in Figure with a yellow mask.

Additionally, we utilized MobileSAM~\cite{zhang2023faster}, a lightweight version of the Segment Anything Model (SAM)~\cite{kirillov2023segment} for image segmentation, to generate more accurate pseudo-labels. MobileSAM is a highly generalizable image segmentation model that can provide reasonably precise masks for objects in an image even in zero-shot scenarios, but it cannot provide labels. Leveraging these label-less but precise masks, we can refine inaccurate the boundary regions of pseudo-labels. We applied the last 3k iterations every 10k iterations, resulting in a total of 12k iterations out of 40k iterations. And, we also applied the attaching the private class from the target to source in OpenReMix only when pseudo-label refinement using MobileSAM was applied.

% We applied pseudo-label refinement using MobileSAM. Multiple masks are generated through MobileSAM, and for each mask, the corresponding pseudo label is filled with the class that occupies the largest proportion. Applied 3k iterations for each of the last 10k iterations, totaling 12k iterations out of a total of 40k iterations. after applying Classmix~\cite{olsson2021classmix}, one more thing class that has not been subjected to Classmix is selected, resized, and added to a random location in the target image.
%$+8.51\%$

\section{BUS with Other Baselines}
\input{sec/table/supple_main}
In Table~\ref{tab:others}, the experiments involved applying head-expansion to some self-training based UDA methods and adding BUS. It showed that the increase of H-Score for DAF~\cite{hoyer2022daformer} by $+8.29\%$ and for HRDA~\cite{hoyer2022hrda} by $+9.19\%$, performance improvement even when applying BUS to other self-training based UDA methods. Particularly, in the case of MIC~\cite{hoyer2023mic}, there was a substantial increase of $+18.02\%$. Furthermore, the higher the performance of the UDA model, the more significant the performance gap when applying BUS. This is because DECON loss and the attaching the private class from the target to the source in OpenReMix benefit from being applied with an accurate target private map. Therefore, models that generate more accurate pseudo-labels have an advantage.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{8.pt}
\begin{tabular}{c|c|c|c|c|c}
%\hline
\specialrule{1.5pt}{0.1pt}{0pt}
$\tau_p$     & 0.3   & 0.4   & \textbf{0.5}   & 0.6   & 0.7   \\ \hline
H-Score & 17.91 & 32.21 & \textbf{61.81} &26.74  & 23.36 \\ \hline
%\hline
\specialrule{1.0pt}{0.1pt}{1pt}
\end{tabular}%
}
\vspace{-2mm}
\caption{\label{tab:threshold} Sensitivity of threshold, denoted as $\tau_p$, for assignment to unknown classes during pseudo labeling on GTA5 $\rightarrow$ Cityscapes.}
\end{table}


\section{Sensitivity of Threshold for Pseudo-Label}
We studied the influence of threshold $\tau_p$ for assignment to unknown classes during pseudo labeling. Table ~\ref{tab:threshold} shows the experimental results for various values of $\tau_p$ on GTA5 $\rightarrow$ Cityscapes. It is observed that for any value other than $\tau_p=0.5$, the performance degrades significantly. Therefore, our method is very sensitive to $\tau_p$, so selecting an appropriate threshold is very important.

\section{More Experiments about Unknown Proportion}
In the main paper, we demonstrated improved performance even when reducing the number of unknown classes compared to the baselines. Table~\ref{tab:numof_unknown_up} presents the comparison results with baselines when the number of unknown classes increased. For 8 unknown classes, we included (``M.bike", ``Bike"), and for 10 unknown classes, we additionally added (``Light", ``Bus"). Despite an increase in the number of unknown classes, our method continues to outperform the baselines.

\input{sec/figure/OpenReMix}

\begin{table}[t]
\vspace{0.3mm}
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{10.pt}
\renewcommand{\arraystretch}{1.2}
\begin{NiceTabular}{c|c|c|c}
\specialrule{1.5pt}{0.1pt}{0pt}
% \hline
\multicolumn{4}{c}{\textbf{GTA5} $\rightarrow$ \textbf{Cityscapes}}           \\ \hline
\multicolumn{1}{c}{\# of Unknown} \vline & Config. A & Config. B & \textbf{Ours}  \\ \hline
\multicolumn{1}{c}{6}       \vline      & 19.71          & 43.79              & \multicolumn{1}{c}{61.81} \\
\multicolumn{1}{c}{8}       \vline      &   20.06        &        52.76       & \multicolumn{1}{c}{62.01} \\
\multicolumn{1}{c}{10}       \vline      &   18.89         &        48.88       & \multicolumn{1}{c}{54.19} \\

\specialrule{1.5pt}{0.2pt}{1pt}
% \bottomrule
\end{NiceTabular}%
}
\vspace{-2mm}
\caption{\label{tab:numof_unknown_up} The comparison of the number of unknown classes. Config. A denotes confidence-based MIC and config. B denotes MIC with head-expansion.}
%  Unknown 갯수에 따른 실험
\end{table}





\section{Influence of DECON Loss Parameters}
\subsection{Crop Size of Private Map}
Table~\ref{tab:crop_size} shows experimental results on the effect of random crop size applied to the target private map. In terms of the H-Score, the best performance was observed at a size of 64$\times$64. However, at 32$\times$32, there is a very slight gap of $0.39\%$. On the other hand, at 128$\times$128, the performance decreased by a larger $1.12\%$. This is because, with larger crop sizes, there is a higher likelihood of including inaccurate target private maps, especially at boundaries of common classes where confidence scores are low.


\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{12.5pt}
%\renewcommand{\arraystretch{1.}}
\begin{tabular}{c|ccc}
\specialrule{1.5pt}{0.1pt}{0pt}
Crop Size & Common & Private & H-Score \\ \hline
$128 \times 128$                  & 71.66           & 52.64            & 60.69            \\
\textbf{64 $\times$ 64}                & 72.33           & \textbf{53.95}            & \textbf{61.81}    \\
$32 \times 32$               &   \textbf{72.87}              &   53.08               &   61.42               \\ 
\specialrule{1.5pt}{0.2pt}{1pt}
%\hline
\end{tabular}%
}
\vspace{-2mm}
\caption{\label{tab:crop_size} Influence of random crop size on the target private map for DECON loss on GTA5 $\rightarrow$ Cityscapes.}
\end{table}


\subsection{Kernel Size of Dilation and Erosion Functions}
We examined the influence of kernel sizes when applying dilation and erosion functions to the target private map. In Table ~\ref{tab:kernel_size}, as we sequentially increased the size from $3 \times 3$  to $7 \times 7$, it showed that not only the H-Score but also the performance of common and private gradually decreased. We hypothesized that the reason for this result is that, with larger kernel sizes, common class regions that are farther away from the boundary of the target private are included. Consequently, the model is less able to focus on distinguishing common and private at the boundary compared to smaller kernel sizes.






\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{10.5pt}
\begin{tabular}{c|ccc}
\specialrule{1.5pt}{0.1pt}{0pt}
Kernel Size & Common & Private & H-Score \\ \hline
\textbf{3 $\times$ 3}                  & \textbf{72.33}           & \textbf{53.95}            & \textbf{61.81}            \\
$5 \times 5$                  & 72.12           & 52.09            & 60.49            \\
$7 \times 7$                  & 71.80           & 49.97            & 58.93            \\

\specialrule{1.5pt}{0.2pt}{1pt}
%\hline
\end{tabular}%
}
\vspace{-2mm}
\caption{\label{tab:kernel_size} Influence of kernel sizes when applying dilation and erosion functions to the target private map on GTA5 $\rightarrow$ Cityscapes.}
\end{table}

\section{Influence of Scale Factor for Resizing Object}
Table ~\ref{tab:resize_scale} shows the experimental results on the effect of the scale factor, denoted as $s_r$, for the resizing object from the source. In cases where 
$s_r>1$, there is a possibility of objects being truncated and pasted to the target. The best Private and H-Score are observed when $s_r=0.5$.
When $s_r=2$, the performance of Common is the best, as the proportion of the common class increases. $s_r=0.75$ and $s_r=1.5$ cases show a significant decrease in performance compared to $s_r=0.5$. This implies that selecting an appropriate $s_r$ is important. 

\section{Further experiments in another domain}

\section{Comparison with BUDA}
We respectfully disagree that BUDA is a super-set of OSDA-SS.
In BUDA, models have access to \emph{private category definitions}, a crucial assumption not shared by OSDA-SS.
In our OSDA-SS setting, there is no provision for such private category definitions. 
We believe both OSDA-SS and BUDA settings have their merit.
In OSDA-SS, one should devise a method that \emph{rejects} novel classes without needing to know any information about their definition.
In BUDA, one should devise a method that \emph{predicts} novel classes explicitly \emph{at the expense of} predefined class definitions. We maintain that our work pioneers the OSDA-SS task. Given the fundamental differences between OSDA-SS and BUDA, direct comparison is not practical. Nonetheless, we offer a comparative analysis in Table~\ref{tab:BUDA_experiment}. Please note that BUDA has the \emph{privilege to access novel class definitions} while BUS and MIC do not.
\section{What if using \textbf{(}$\mathbf{\textit{C}+\textit{N}}$\textbf{)} heads?}
In our OSDA-SS task, the number of private classes $N$ is unknown since target private labels are absent. In that sense, setting $N=1$ for the private class is a reasonable option. Despite this, we experimented using $(C+N)$ heads with random pseudo-labeling. Understandably, Table~\ref{tab:N_C_Head} demonstrates that our BUS shows the best performance when $N$ is set to 1.


\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{10.5pt}
%\renewcommand{\arraystretch}{0.8}
{\scriptsize
\begin{tabular}{c|ccc}

\specialrule{1.0pt}{0.1pt}{0pt}
\textbf{$s_r$} & Common      & Private     & H-Score     \\ \hline
2                  & \textbf{72.58}                     &     48.48                 &  58.13             \\ 
1.75               & 72.17                     & 50.93                      & 59.72                     \\
1.5                & 72.42                     &      44.90                &         55.14             \\
1.25               &  71.29                    &  52.16                    & 60.24                     \\
%1                  &                    &                           &  \\
0.75               & 68.54              & 48.65                     & 56.91 \\
\textbf{0.5}                & 72.33           & \textbf{53.95}            & \textbf{61.81}               \\
0.25               & 71.98 & 50.74 &  59.52\\ 
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
}
\vspace{-2mm}
\caption{\label{tab:resize_scale} Influence of scale factor, denoted as $s_r$, for resizing object from source on GTA5 $\rightarrow$ Cityscapes.}
\end{table}

\end{appendix}




\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{10.5pt}
\renewcommand{\arraystretch}{1.0}
{\scriptsize
\begin{NiceTabular}{l|c|c}
%\hline
\specialrule{1.5pt}{0.1pt}{0pt}
\multicolumn{1}{c|}{$s_r$}                    & GTA5 $\rightarrow$ Cityscapes & SYNTHIA $\rightarrow$  Cityscapes \\ \hline
\textbf{[}$\mathbf{0.5,0.5}$\textbf{]}           & \textbf{61.81}              & \textbf{41.49} \\ \dashedline

$[0,2]$ (All)          & 59.73              & 36.77                 \\
$[1,2]$ (Upscale)   & 54.36              &   37.73               \\
$[0,1                                              
                                                   
 ]$ (Downscale) & 59.84              &  38.90                \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{NiceTabular}%
}
}
\vspace{-4mm}
\caption{\label{tab:random_resize_scale} Influence of the scale factor, denoted as $s_r$.}
\vspace{-4mm}
\end{table}

%\end{document}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{25.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc>{\columncolor[gray]{0.9}}c}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
Method       & Common        & Private       & H-Score       \\ \hline
BUDA         & 37.3          & 18.5          & 24.7          \\
MIC          & 54.3          & 24.1          & 34.4          \\
\textbf{BUS} & \textbf{55.6} & \textbf{39.7} & \textbf{46.3} \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
%\caption{\label{tab:BUDA_experiment} Comparison of BUS with BUDA on private classes 'auto rickshaw' and 'animal'.}
\caption{\label{tab:BUDA_experiment} Additional experiments including BUDA on CS $\rightarrow$ IDD.}%Comparison of BUS with BUDA.}
\vspace{-4mm}
\end{table}



\begin{table}[t]
\centering
\setlength{\tabcolsep}{18.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
%\hline
\specialrule{1.5pt}{0.1pt}{0pt}
$N$     & \textbf{1}   & 3     & 6   & 10   \\ \hline
H-Score & \textbf{61.81} & 46.02 &  38.01 & 30.56 \\ \hline
%\hline
\specialrule{1.0pt}{0.1pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
\caption{\label{tab:N_C_Head} Influence of the number of expansion head dimensions.}
\vspace{-5mm}
\end{table}


==> sec/0_abstract.tex <==
\begin{abstract}
Unsupervised domain adaptation (UDA) for Semantic segmentation aims to transfer the pixel-wise knowledge from the labeled source domain to an unlabeled target domain. However, current UDA methods typically assume a shared label space between source and target, limiting their applicability in real-world scenarios where novel categories may emerge in the target domain. In this paper, we introduce Open Set Domain Adaptation for Semantic Segmentation (OSDA-SS) for the first time, where the target domain includes unknown classes. We identify two major problems in the OSDA-SS scenario as follows: 1) the existing UDA methods struggle to predict the exact boundary of the unknown class, and 2) they fail to accurately predict the shape of the unknown class. To address these issues, we propose \textbf{B}oundary and \textbf{U}nknown \textbf{S}hape-Aware open set domain adaptation, coined \textbf{BUS}. Our BUS can accurately discern the boundaries between known and unknown classes using a novel dilation-erosion-based contrastive loss, which helps to discriminate the region for the unknown class in a contrastive manner. In addition, we propose OpenReMix, a new domain mixing augmentation method that guides our model to effectively learn domain and size-invariant features for improving the shape detection of the known and unknown classes. Through extensive experiments, we demonstrate that our proposed BUS effectively detects the unknown class in the challenging OSDA-SS scenario, compared to the previous methods by a large margin. The code will be publicly released after the review.

\end{abstract}

==> sec/1_intro.tex <==

\section{Introduction}
\label{sec:intro}

% 메서드~\cite 인용 
% ref{} --> label (figure, graph, section + equation)
% cref{label}: Eq.(1)
% \input{sec/figure/motivation1}

% before revision by Jinwoo
% Semantic segmentation is a fundamental computer vision task, that targets to make dense pixel-level predictions on images. It is a key step in numerous applications, including autonomous driving, human-machine interaction, and augmented reality. In the past decades, deep neural networks have achieved significant progress in semantic segmentation. However, it requires pixel-level annotations on images to achieve satisfying performance, which is laborious and time-consuming. To avoid this burdensome task, existing researchers try to use synthetic but photo-realistic large-scale source datasets such as GTA5~\cite{richter2016playing} and SYNTHIA~\cite{ros2016synthia} with computer-generated annotations. However, due to domain shift, directly adapting the model trained on the source domain causes significant performance degradation on the target domain. Unsupervised Domain Adaptation (UDA)~\cite{tsai2018learning, vu2019advent,melas2021pixmatch,hoyer2022daformer,hoyer2022hrda,hoyer2023mic} approach adapts a model trained from a largely labeled synthetic source domain to an unlabeled real target domain without the additional cost of annotations.

% \begin{figure}[t] %%% t: top, b: bottom, h: here
% \centering
% \includegraphics[width=\columnwidth]{sec/figure/motivation_fig1.png}
% \caption{Motivation Figure (purpose): existing approaches (b,c) cannot classify unknown classes (ex. pedestrian). Ours good.}
% \vspace{-5mm}
% \label{fig:longa}
% \end{figure}

%  However, existing UDA methods assume that the source and target domains share an identical label set (closed-set). In real-world scenarios, the target domain may include unknown classes for which labels are absent in the source domain (open-set). In this case, the UDA method does not recognize the existence of unknown classes during training, which can lead to serious consequences (e.g., not recognizing an unknown person and predicting it as a road). Therefore, distinguishing between unknown and known classes during training is crucial. Despite related research existing for the Classification task~\cite{saito2018open, bucci2020effectiveness, jang2022unknown, you2019universal}, there is a lack of studies in Semantic Segmentation tasks. Hence, we propose Open Set Domain Adaptation for Semantic Segmentation (OSDA for SS) to enable Semantic Segmentation models to distinguish unknown classes at the pixel-level.

% We first examined the problems with Unsupervised Domain Adaptation (UDA) that does not consider unknown classes. We devised two naive approaches using confidence scores to predict 'unknown' to adapt them to the OSDA for SS setting.1) During inference, pixels with low confidence scores are assigned to the unknown class, as illustrated in Fig.~\ref{fig:longa}(b). 2) To facilitate the learning of unknown classes in the target domain, we modified the output probability dimension of the model, changing it from $C$ to $C+1$, where $C$ represents the number of known classes. and, during the creation of pseudo-labels for the target, pixels with low confidence scores are designated as the unknown class. The model trains with these newly generated pseudo-labels as illustrated in Fig.~\ref{fig:longa}(c). Despite employing these two methods, the model can predict 'unknown' to some extent. However, challenges persist in accurately capturing the shape of unknown classes and avoiding confusion between known and unknown classes.

% Therefore, we propose three methods to address the problems. First, dilation mask based loss for known/unknown discrimination with emphasis on the boundary. Semantic Segmentation models, especially at the boundaries of classes, exhibit a propensity for confusion in predictions~\cite{liu2021bapa,caliva2019distance,li2020improving}. The absence of label information for unknown classes further exacerbates the difficulty in predicting at these boundary regions. Therefore, if the model can definitively distinguish between known and unknown classes at the ambiguous boundaries of the unknown class, it would enhance the precision of predicting unknown classes and enable the accurate prediction of their shapes.
% %
% Second, Classmix~\cite{olsson2021classmix} with resizing for shape of unknown class, If the model accurately predicts despite variations in the size of classes, it can effectively capture the shape of the classes. Additionally, a robust understanding of the shape of known classes enables effective knowledge transfer for capturing the shape of unknown classes. Unlike Classmix~\cite{olsson2021classmix}, which overlays specific classes from the source onto the target, our approach involves resizing source object classes for additional overlay. This not only facilitates learning domain-invariant representations but also size-invariant representations.
% %
% Third, Bi-Mix for efficiently learning unknown classes, During the training process, when learning from source images, the additional $C+1$ output probability dimension is not utilized as there are no unknown classes present in the ground truth of the source. To efficiently utilize this dimension, we employ an approach opposite to Classmix~\cite{olsson2021classmix}. Instead of overlaying specific classes from the source onto the target, we overlay the unknown class from the target onto the source. This way, The model trains on images where the source and unknown classes are from the target image. The unknown class region is extracted based on the pseudo-labels from the target. This approach allows the model to train on a more substantial quantity of unknown classes, improving the model's ability to predict unknown classes more effectively.

% The contributions of this paper can be summarized as follows:

% \begin{itemize}
% \item We explain the necessity of Open-Set Domain Adaptation for semantic segmentation (OSDA for SS) tasks, and attempt to solve the OSDA for SS scenario the first time to the best of our knowledge.

% \item We introduce a dilation mask-based loss. The method utilizes a target private class mask map and dilation and erosion techniques to better discriminate between common and private classes, especially at the boundary.


% \item We propose two domain mixing techniques. Classmix with resizing for learning size-invariant representations, and Bi-Mix for learning more unknown classes.


% \item Experimentally, we demonstrate that our approach is state-of-the-art by comparing it to unsupervised domain adaptation for semantic segmentation and open domain adaptation for classification methods.

% \end{itemize}

% after revision by Jinwoo
In semantic segmentation, a model predicts pixel-wise category labels given an input image. Semantic segmentation has a lot of applications, \eg, autonomous driving~\cite{geiger2012we}, human-machine interaction~\cite{tsai2017deep}, and augmented reality. Over the past decade, there has been notable advancement in supervised semantic segmentation driven by deep neural networks~\cite{long2015fully,yu2015multi,chen2017deeplab,xie2021segformer}. However, supervised semantic segmentation requires pixel-level ground truth annotations, which are labor-intensive and costly. To mitigate the annotation challenges, unsupervised domain adaptation (UDA) has emerged~\cite{tsai2018learning, vu2019advent,melas2021pixmatch,hoyer2022daformer,hoyer2022hrda,hoyer2023mic}. In the UDA setting, we can leverage the already-labeled source data to achieve high performance on the unlabeled target data. Notably, synthetic datasets for semantic segmentation such as GTA5~\cite{richter2016playing} and SYNTHIA~\cite{ros2016synthia} with annotations automatically generated by game engines present valuable resources for semantic segmentation research.

% \begin{figure}[t] %%% t: top, b: bottom, h: here
% \centering
% \includegraphics[width=\columnwidth]{sec/figure/motivation_fig1.png}
% \caption{Motivation Figure (purpose): existing approaches (b,c) cannot classify unknown classes (ex. pedestrian). Ours good.}
% \vspace{-5mm}
% \label{fig:longa}
% \end{figure}

\begin{figure}
\centering
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{sec/figure/motivation_figure1/motive1_a.png}
    \caption{Ground truth.}
    \label{fig:1}
  \end{subfigure}
 \vfill
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{sec/figure/motivation_figure1/motive1_b.png}
    \caption{UDA method (MIC~\cite{hoyer2023mic}).}
    \label{fig:2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{sec/figure/motivation_figure1/motive1_c.png}
    \caption{Confidence-based threshold.}
    \label{fig:3}
  \end{subfigure}
 \vfill
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{sec/figure/motivation_figure1/motive1_d.png}
    \caption{\small{Unknown head expansion.}}
    \label{fig:4}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[width=\textwidth]{sec/figure/motivation_figure1/motive1_e.png}
    \caption{BUS (\textbf{Ours}).}
    \label{fig:5}
  \end{subfigure}
 % \hfill
 %  \begin{subfigure}[b]{0.48\columnwidth}
 %    \includegraphics[width=\textwidth]{example-image}
 %    \caption{Picture 6}
 %    \label{fig:6}
 %  \end{subfigure}
\caption{Visualization of prediction maps in the OSDA-SS scenario. Here, the pixels detected by the white color mean the unknown class. The naive UDA method (b) is completely unaware of the \emph{unknown} class. Even after applying simple techniques to help the UDA model recognize the \emph{unknown}, we can see that it still struggles to accurately predict the shape of the \emph{unknown}, as shown in examples (c) and (d).}
\label{fig:motiv}
\end{figure}


UDA methods typically presume that source and target datasets share the same label space. Such an assumption is not reasonable in real-world applications. In the target data, novel categories not presented in the source dataset (target-private categories) may emerge, leading to an Open Set Domain Adaptation (OSDA) setting. The conventional UDA method may significantly fail under OSDA setting, \eg a model may erroneously label a person walking on the road as the road itself as shown in \figref{motiv} (b). The desired model should reject any target-private class as \emph{unknown} rather than misclassifying it as a known class. While OSDA has been explored in image classification~\cite{saito2018open, bucci2020effectiveness, jang2022unknown, you2019universal}, its application to semantic segmentation remains unexplored to the best of our knowledge. In this work, we tackle the interesting and challenging problem of Open Set Domain Adaptation for Semantic Segmentation (OSDA-SS). Here, we deal with labeled source data and unlabeled target data containing classes not found in the source. In OSDA-SS, the goal of a model is to accurately predict pixel-wise category labels in the target domain and correctly identify any unseen classes during training as \emph{unknown}.

One can design reasonable baselines by extending well-established UDA methods. One approach could be a confidence-threshold baseline. We train a model by using any UDA algorithm without considering target-private classes. During inference, the model labels pixels with confidence scores below a set threshold as \emph{unkown}. We show the output segmentation map of the confidence-threshold baseline in \figref{motiv} (c). Another baseline could be a head-expansion baseline. We expand the classification head from $C$ to $(C+1)$ dimensions, where $C$ represents the number of known classes. We train the baseline with pseudo-labeling and confidence thresholding. We assign \emph{unknown} pseudo-label to pixels with a confidence lower than a threshold. We show the output segmentation map of the baseline in \figref{motiv} (d). The baselines sometimes reject target-private classes as \emph{unknown}. However, the baselines often fail to reject target-private classes which results in poor performance on the target dataset.

In this work, we build a model upon the head-expansion baseline. We find two failure modes of the baseline and propose a novel \textbf{B}oundary and \textbf{U}nknown \textbf{S}hape-Aware (\textbf{BUS}) OSDA method addressing them. 
First, semantic segmentation models are often less confident or even fail near the boundaries of objects~\cite{liu2021bapa,caliva2019distance,li2020improving}. We find that the problem is even more severe for target-private classes due to lack of supervision. To address this issue, we propose a new \textbf{D}ilation-\textbf{E}rosion-based \textbf{CON}trastive (\textbf{DECON}) loss that manifests the boundaries through morphological operations, specifically dilation and erosion. 
% Given a target image, we generate a target-private map by pseudo-labeling with the expanded head. 
% Subsequently, we apply dilation and erosion separately to generate dilation and erosion maps from the private map. 
% In the dilation map, subtracting the private map manifests known class regions near the boundaries. 
% Conversely, the erosion map manifests regions that are definitively private classes. 
Given a target image, we generate a target-private map by pseudo-labeling with the expanded head. 
Subsequently, we generate a boundary map by subtracting the original private map from the dilated private map, indicating \emph{known} class regions near the boundaries.
We generate an erosion map by applying erosion to the private map, indicating more confident \emph{private class} regions.
We then use the features from the erosion map as positive samples and the boundary map as negative samples. With DECON, our model can clearly discern the boundaries between common and private classes.

Second, the baseline model faces challenges in accurately predicting the shape of \emph{unknown}. If the model consistently predicts the same object regardless of variations in size, it indicates that the model relies more on shape information than size information to recognize the object. Inspired by this motivation, we propose a new data mixing augmentation, \textbf{OpenReMix}. This method involves 1) resizing a thing class from the source and mixing it with the target during training, aiming to train the model to consistently predict the same object even when its size varies. In addition, since there is no \emph{unknown} class in the source, 2) we cut \emph{unknown} objects from a target image and paste them into a source image for supplemental learning of the last (C+1)-th head, aiding in the rejection of \emph{unknown} during source training. This delicate mixing strategy notably enhances the detection capability of \emph{unknown}, with a specific emphasis on capturing the shape information. By addressing the failure modes, the proposed BUS achieves significant performance gains on public benchmarks: GTA5$\rightarrow$Cityscapes and GTA5$\rightarrow$SYNTHIA.
% \eg $+23.01$ in GTA5-to-Cityscapes, and $+20.67$ in SYNTHIA-to-Cityscapes.

We summarize our major contributions as follows:
\begin{itemize}
\item To the best of our knowledge, we introduce a new task, Open Set Domain Adaptation for Semantic Segmentation (OSDA-SS) for the first time. To tackle this challenging task, we propose a novel \textbf{B}oundary and \textbf{U}nknown \textbf{S}hape-Aware OSDA method, coined \textbf{BUS}.

\item We introduce DECON, a new dilation-erosion-based contrastive loss to address the less confident and wrong predictions near the class boundaries.

\item We propose OpenReMix, which leads our model to learn size-invariant features and leverages \emph{unknown} objects from target to source to train the expanded head efficiently. OpenReMix encourages our model to focus on shape information of \emph{unknown}.

\item We conduct extensive experiments to validate the effectiveness of our proposed method. The proposed BUS shows state-of-the-art performance on public benchmark datasets with a significant margin.

\end{itemize}
%-------------------------------------------------------------------------




==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_prior.tex <==
\section{Related Work}
\label{sec:related}


% \paragraph{Semantic segmentation.}
\subsection{Semantic Segmentation.}

% before revision by Jinwoo
% Semantic segmentation aims to predict regions of different semantic categories at pixel level for a given images. Fully Convolutional Netowrks (FCNs)~\cite{long2015fully} is a classic semantic segmentation network and has achieved impressive performance. However, they have relatively small receptive field to explore the global context of the image. To better represent the context, many later works focus on dilated convolution~\cite{chen2017deeplab,yu2015multi}, global pooling~\cite{liu2015parsenet}, pyramid pooling\cite{zhao2018icnet,zhao2017pyramid,yang2018denseaspp}, and attention mechanism ~\cite{fu2019dual,huang2019ccnet,zhao2018psanet,zhu2019asymmetric}. Despite the success, these semantic segmentation networks have a problem that their performance is significantly poor for unseen domains due to domain shift problem. To this end, many domain adaptation methods are proposed to provide good performance for unseen domains even if domain shift occurs by reducing domain gap.

% after revision by Jinwoo
Semantic segmentation, which is a task to predict pixel-wise labels from input images, has witnessed significant advances over the last decade. 
%
Key developments include fully convolution networks (FCNs)~\cite{long2015fully}, dilated convolution~\cite{chen2017deeplab,yu2015multi}, global pooling~\cite{liu2015parsenet}, pyramid pooling~\cite{zhao2018icnet,zhao2017pyramid,yang2018denseaspp}, and attention mechanism ~\cite{fu2019dual,huang2019ccnet,zhao2018psanet,zhu2019asymmetric}. 
%
Despite their success, these methods typically depend on a large amount of labeled data which is label-intensive and costly.
%
In contrast, we formulate the semantic segmentation problem as domain adaptation to mitigate the annotation cost.


% \paragraph{Unsupervised domain adaptation for semantic segmentation.}
\subsection{Unsupervised Domain Adaptation for Semantic Segmentation.}
% before revision by Jinwoo
% The goal of Unsupervised Domain Adaptation (UDA) is to bridge the domain gap by transferring the knowledge from the labeled source domain to the unlabeled target domain. UDA is an important task for semantic segmentation because it can efficiently solve the cost problem of per-pixel annotation. The general ideas for UDA semantic segmentation include adversarial learning~\cite{hong2018conditional,kim2020learning,pan2020unsupervised,tsai2018learning,tsai2019domain,chen2019synergistic,du2019ssf} and self-training strategy~\cite{Zou_2018_ECCV,chen2019domain,zou2019confidence,wang2021domain,lian2019constructing,li2019bidirectional,Wang_2021_ICCV,melas2021pixmatch,zhang2021prototypical,tranheden2021dacs,hoyer2022daformer,hoyer2022hrda,hoyer2023mic}. We briefly review some recent works. First, adversarial learning-based methods employ a discriminator network. A segmentation network generates the segmentation maps of the different domains, and the discriminator network is trained to predict the domain between the source and target domain. The segmentation network aims to fool the discriminator. Then, it ensures that the features of two domains have a similar distribution. In recent years, self-training methods show significant performance improvement in UDA. The self-training approach generates the segmentation map of the given target image, and obtains pseudo labels by collecting only the results of pixels whose confidence score exceeds a certain threshold. The generated pseudo labels then iteratively re-train the model with both the ground truth of source domain and pseudo labels of target domain. At this time, since the quality of the pseudo labels is very crucial, there are various studies to refine the noisy pseudo labels.However these research is primarily conducted in a closed-set setting, assuming complete alignment of label sets between the source and target domains.In real-world scenarios, the absence of labels for the target makes it challenging to confirm whether it is a closed setting, thereby constraining its applicability.

% after revision by Jinwoo
Recently, there has been a lot of work on unsupervised domain adaptation (UDA) for semantic segmentation.
%
UDA methods for semantic segmentation generally fall into two categories: adversarial learning-based and self-training approaches.
%
Adversarial learning-based UDA methods~\cite{hong2018conditional,kim2020learning,pan2020unsupervised,tsai2018learning,tsai2019domain,chen2019synergistic,du2019ssf} utilize an adversarial domain classifier to learn domain-invariant representations, aiming to deceive the domain classifier.
%
Self-training methods~\cite{Zou_2018_ECCV,chen2019domain,zou2019confidence,wang2021domain,lian2019constructing,li2019bidirectional, Wang_2021_ICCV,melas2021pixmatch,zhang2021prototypical,tranheden2021dacs,hoyer2022daformer,hoyer2022hrda,hoyer2023mic} create pseudo segmentation labels for each pixel in the target domain image by confidence thresholding. 
%
Then self-training methods iteratively re-train models, which results in the enhanced performance on the target domain.
%
Despite the great success, most previous works assume a closed set setting, where the source and target domains share the same label space.
%
In this work, we relax this unrealistic assumption and tackle the problem of open set domain adaptation for semantic segmentation (OSDA-SS). 
%
To the best of our knowledge, there is no prior work to tackle this problem.


% \paragraph{Open Set Domain Adaptation}
\subsection{Open Set Domain Adaptation}

Open set domain adaptation (OSDA) extends UDA to handle novel categories in the target domain that are not present in the source domain. The primary goal of OSDA is to effectively distinguish between known and unknown categories while reducing the domain gap between the known classes in the source and target domains. OSDA evolves through the use of techniques such as adversarial learning~\cite{saito2018open, liu2019separate} and pseudo-labeling~\cite{wang2021progressively,jang2022unknown,mei2020instance} for classification. However, in semantic segmentation tasks, which require a higher degree of spatial information compared to classification, existing methods struggle to effectively differentiate unknown categories. To address this challenge, we propose an approach for semantic segmentation tasks to discriminate unknown categories.

\subsection{Domain Mixing Augmentation.}
To improve the generalization power of deep neural networks, mixup~\cite{zhang2017mixup,tokozume2018between} and its variants~\cite{olsson2021classmix,yun2019cutmix,french2020milking,tranheden2021dacs,gao2021dsp,berthelot2019mixmatch,french2019semi,na2021fixbi,wu2020dual,xu2020adversarial} have been proposed.
%
Especially, domain mixing augmentation demonstrates significant performance improvement in UDA~\cite{olsson2021classmix,yun2019cutmix,french2020milking,tranheden2021dacs,gao2021dsp, chen2022deliberated} by utilizing domain-mixed images as training data to encourage the learning of domain-invariant feature representations.
%
We propose OpenReMix for the challenging OSDA-SS scenario by encouraging our model to capture shape information, especially for the \emph{unknown} class.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_overview.tex <==
%\section{Preliminary}
%\label{sec:overview}


%\subsection{Problem definition}
%We have a source domain image \(x_i^s \in \mathbb{R}^{3 \times H \times W}\) and the corresponding pixel-wise vectors \(y_i^s \in \mathbb{B}^{C \times H \times W}\) sampled from the set of source images \(X^s\) and the source label set \(Y^s\).
%Here, \(i\) refers to the \(i\)-th sample, \(H\) and \(W\) are the height and width of the image, respectively, and \(C\) denotes the number of categories.
%In the target domain, we only have an image \(x_i^t \in \mathbb{R}^{3\times H \times W}\) without the corresponding label \(yi^t\).
%The source and target domains share \(C\) categories, and the target domain has an additional unknown class. Our goal is to train a segmentation model using both the labeled source data \((x^s, y^s) \in X^s\times Y^s\) and the unlabeled target data \(x^t \in X_i^t\), which performs well in known and unknown classes on the target domain.



==> sec/4_method.tex <==


\input{sec/figure/fig_main}

\section{Method}
\label{sec:Method}

\subsection{Problem Formulation}
%\label{sec:problem}
% We have the labeled source domain data as $S=\left\{(x_1^s,y_1^s ),…  ,(x_N^s,y_N^s )\right\}$, as well as unlabeled target domain data as $T=\left\{(x_1^t),…  ,(x_N^t)\right\}$. $x_i^s\in R^{3\times H \times W}$ and $y_i^s\in \left\{0,1\right\}^{H\times W}$ represent the source image and the corresponding pixel-wise annotation. Then, $H$ and $W$ are height and width of the image, and $C$ is the number of classes. Our goal is to train a segmentation model on $S$ and $T$ and evaluate on the target domain. The source and target domains share the same $K$ classes. Generally, the segmentation model consists of a feature extractor $F$ and a classifier $C$, which predicts pixel-wise predictions for an image.
%We have a source domain image $X^s \in \R^{3\times H \times W}$ and the corresponding pixel-wise one-hot vectors $Y^s \in \B^{K \times H \times W}$ sampled from the set of source images $X^s$ and the source label set $Y^s$.
%In contrast to traditional MIC methods, which generate pseudo-labels only for known classes, our approach to pseudo-label generation involves assigning an unknown label to pixels with confidence below a set threshold.

In this section, we formulate a novel OSDA-SS task for the first time. In OSDA-SS, a network is trained with the source images \(X_s\)$=\{x_s^1, x_s^2, ..., x_s^i\}$ and the corresponding labels \(Y_s\)$=\{y_s^1, y_s^2, ..., y_s^i\}$ to ensure effective performance in the target domain \(X_t\)$=\{x_t^1, x_t^2, ..., x_t^i\}$ without labels.
\(x_s^i \in \mathbb{R}^{3 \times H \times W}\) and \(y_s^i \in \mathbb{R}^{C \times H \times W}\) are the \(i\)-th source domain image and the \(i\)-th pixel-wise label. 
\(H\) and \(W\) are the height and the width of the image, respectively, and \(C\) denotes the number of categories in source domain. In the target domain, we only have an image \(x_t^i \in \mathbb{R}^{3\times H \times W}\) without the corresponding labels. The source and target domains share \(C\) categories, and the target domain has an additional unknown class, \textit{i.e.}, the target images contain unknown objects. In this setting, the goal of OSDA-SS is to train a segmentation model \(f_\theta\) using both the labeled source data $(X_s, Y_s)$ and the unlabeled target data \(X_t\), and eventually the learned model \(f_\theta\) should predict both known and unknown classes well on the target domain.

% a source domain image \(x_s^i \in \mathbb{R}^{3 \times H \times W}\) and the corresponding pixel-wise labels \(y_s^i \in \mathbb{R}^{C \times H \times W}\) sampled from the set of source images \(X_s\) and the source label set \(Y_s\).Here, \(i\) refers to the \(i\)-th sample, \(H\) and \(W\) are the height and width of the image, respectively, and \(C\) denotes the number of categories.In the target domain, we only have an image \(x_t^i \in \mathbb{R}^{3\times H \times W}\) without the corresponding label \(y_t^i\).The source and target domains share \(C\) categories, and the target domain has an additional unknown class. Our goal is to train a segmentation model \(f_\theta\) using both the labeled source data \(X_s, Y_s\) and the unlabeled target data \(X_t\), which predicts well in both known and unknown classes on the target domain.

\subsection{Baseline}
Inspired by the UDA methods based on self-training~\cite{tranheden2021dacs,hoyer2022daformer,hoyer2022hrda,hoyer2023mic}, we build a simple OSDA baseline by extending the number of classifier heads from $C$ to $(C+1)$, where the $(C+1)$-th head corresponds to an \emph{unknown} class. The segmentation network \(f_\theta\) then trains the labeled source domain using the following categorical cross-entropy loss $\mathcal{L}_{seg}^{s}$:
\begin{align}
\mathcal{L}_{seg}^{s} = -\sum_{j=1}^{H \cdot W}\sum_{c=1}^{C+1} {y}_{s}^{(j,c)} \log f_\theta(x_{s})^{(j,c)},
\label{eq:source_cleanloss}
\end{align}
where $j \in \{1, 2, ..., H \cdot W\}$ denotes the pixel index and $c \in \{1, 2, ..., C+1\}$ denotes the class index. For the target domain, to alleviate the domain gap between the source and the target, the baseline utilizes a teacher network \(g_\phi\) on the target to generate pseudo-labels. The pseudo-label $\hat{y}_{tp}^{(j)}$ for the $j$-th pixel considering \emph{unknown} can be acquired as follows:
\begin{align}
\hat{y}_{tp}^{(j)} = 
\begin{cases} 
c', & \text{if } \left( \max_{c'}g_\phi(x_t)^{(j,c')} \geq \tau_p \right) \\
C+1, & \text{otherwise}
\end{cases}
,
\end{align}
where $c^{'} \in C$ denotes a class belonging to known classes $C$, and $\tau_p$ is a threshold. Using the above equation, we assign the pixels as the \textit{unknown} class when the maximum softmax probability is lower than $\tau_p$.

Since we cannot completely trust the pseudo-labels above, we estimate the confidence of the pseudo-label by utilizing the ratio of pixels~\cite{tranheden2021dacs}. To this end, we count the number of pixels that have the maximum probability values exceeding a certain threshold \(\tau_t\) as follows:
\begin{align}
q_t = \frac{1}{H \cdot W} \sum_{j=1}^{H \cdot W} \left[ \max_{c'} g_\phi(x_t)^{(j, c')} \geq \tau_t \right],
%q_t^{j} = \frac{1}{H \cdot W} \sum_{j=1}^{H \cdot W} \left[ \max_{c'} g_\phi(x_t)^{(j, c')} \geq \tau_t \right],
\end{align}
where \(q_t^{j}\) means the confidence of the pseudo-label for the $j$-th pixel. The network \(f_\theta\) then trains the target domain using the pseudo-labels and the corresponding confidence estimates using the following categorical cross-entropy loss $\mathcal{L}_{seg}^{t}$:
\begin{align}
\mathcal{L}_{seg}^{t} = -\sum_{j=1}^{H \cdot W}\sum_{c=1}^{C+1} {q_t \hat{y}_{tp}^{(j,c)} \log f_\theta(x_{t})^{(j,c)}}.
%\mathcal{L}_{seg}^{t} = -\sum_{j=1}^{H \cdot W}\sum_{c=1}^{C+1} {q_t^{(j)} \hat{y}_{tp}^{(j,c)} \log f_\theta(x_{t})^{(j,c)}}.
\label{eq:target_loss}
\end{align}

Finally, we update the teacher network \(g_\phi\) from \(f_\theta\) using the exponential moving average (EMA)~\cite{tarvainen2017mean} with a smoothing factor \(\alpha\), where the equation is shown as follows:
\begin{align}
\phi_{t+1} = \alpha \phi_t + (1 - \alpha) \theta_t.
\end{align}


Based on this baseline, we propose a novel \textbf{B}oundary and \textbf{U}nknown \textbf{S}hape-Aware OSDA method, coined \textbf{BUS}, which involves a new loss function to manifest the boundaries of known and unknown classes (see Section \ref{sec:DECON}), and a new domain mixing augmentation to detect the shape of unknown objects robustly (see Section \ref{sec:OpenReMix}).
% Additionally, we introduce an additional DECON Loss to the baseline. Furthermore, we leverage domain mixing data augmentation OpenReMix to train on augmented images instead of the source and target images used in the baseline training process.


%Self-training based on UDA performs well in closed scenarios but fails to recognize unknown classes in open scenarios. To address this limitation, we extend the dimension of the classification head to learn unknown classes, resulting in a modification of the loss term \eqref{eq:source_cleanloss} to
%\begin{align}
%L_{seg}^{sp} = -\sum_{j=1}^{H \cdot W}\sum_{c=1}^{C+1} {y}_{s}^{(j,c)} \log f_\theta(x_{s})^{(j,c)}.
%\label{eq:new_source_cleanloss}
%\end{align}



%The modified target domain loss \eqref{eq:target_loss}, using the updated pseudo-labels, is as follows
%\begin{align}
%L_{seg}^{tp} = -\sum_{j=1}^{H \cdot W}\sum_{c=1}^{C+1} {q_t^{(j)} \hat{y}_{tp}^{(j,c)} \log f_\theta(x_{t})^{(j,c)}}.
%\label{eq:new_target_loss}
%\end{align}
%Additionally, MIC utilizes augmented target data following DACS~\cite{tranheden2021dacs}, incorporates multi-resolution techniques~\cite{hoyer2022hrda}, and includes losses from DAFormer~\cite{hoyer2022daformer}. The final loss is expressed as follows. In our approach, we introduce an additional Dilation-Erosion-Based Contrastive Loss to the baseline. Furthermore, we leverage two domain mixing techniques, Classmix~\cite{olsson2021classmix} with resizing and Bi-Mix, to train on augmented images instead of the original images used in the baseline training process.


\subsection{Dilation-Erosion-based Contrastive Loss}
\label{sec:DECON}
Semantic segmentation models often struggle to confidently predict object boundaries~\cite{liu2021bapa,caliva2019distance,li2020improving}, especially for target-private classes, where the absence of label information makes boundary prediction even more challenging. Moreover, since the segmentation models predict the boundaries with low confidence estimates, the quality of generated pseudo-labels may not be accurate. If the model can confidently differentiate the boundaries between known and unknown classes, accurate predictions of the unknown class shapes become feasible. 

To discern the boundaries effectively, we leverage two morphological operations, which are dilation and erosion. First, we utilize the pseudo-labels from the target to create a target private map as follows: 
\begin{align}
M_{u}^{(i,j)} = 
\begin{cases} 
1, & \text{if } \hat{y}_{tp}^{(i,j)}=C+1 \\
0, & \text{otherwise}
\end{cases},
\label{eq:target_private}
\end{align}
where $i,j$ denoted the pixel index representing the height and width of $\hat{y}_{tp}$.

Next, we apply the dilation function \(h_{d}\) and the erosion function \(h_{e}\) to the randomly cropped target private map, generating dilation and erosion maps. In the dilation map, we additionally subtract the target private map to identify regions associated with the common classes near the boundaries. On the other hand, the erosion map from the boundary emphasizes regions that definitively belong to the private class. We can calculate these maps by the following equations:
\begin{align}
M_{N} &= h_{d}(M'_{u}) - M'_{u} , \\
M_{P} &= h_{e}(M'_{u}),
\end{align}
where $M'_{u}=r(M_{u})$, $r(\cdot)$ is a function of random crop, and \(M_{N}\) and \(M_{P}\) denote the dilation and erosion maps, respectively.

To construct a contrastive loss, we need positive, negative, and anchor samples. To this end, we use dilation and erosion maps since they include regions associated with common and private classes near the boundaries. Therefore, we can obtain each sample as follows:
\begin{align}
z_i&= \mathrm{avg}(M_{P} \odot f_\theta(x_{t})), \\
z_j&=M_{P} \odot f_\theta(x_{t}), \\
z_k&= M_{N} \odot f_\theta(x_{t}),
\end{align}
where $z_i$ is an anchor, $\mathrm{avg}(\cdot)$ denotes the average pooling layer, and $z_j$ and $z_k$ represent positive and negative samples, respectively. We utilize $z_i$ as a prototype calculated by the average of positive samples. Finally, we define the contrastive loss~\cite{chen2020simple} using $z_i$, $z_j$, and $z_k$ as follows:
\begin{align}
%\mathcal{L}_{DECON} =-\log \frac{\exp(\text{sim}(z_i, z_j) / \tau)}{\sum_{k=1}^{N} \mathbbm{1}{[k \neq i]}\cdot \exp(\text{sim}(z_i, z_k) / \tau)}
\mathcal{L}_{DECON} =-\log [{\sum_{p=1}^{N_p} \exp(z_i \cdot z_j^p / \tau)}/{\sum_{n=1}^{N_n} \exp(z_i \cdot z_k^n / \tau)}]
\end{align}
where \(\text{sim}(\cdot, \cdot )\) means cosine similarity, \(\tau\) is a temperature parameter, \textcolor{red}{$N_n$ and $N_p$ denote the number of negative/positive pixels}. To sum up, the proposed $\mathcal{L}_{DECON}$ allows our model to better distinguish between common and private classes near the boundaries.

\subsection{OpenReMix}
\label{sec:OpenReMix}
\paragraph{Resizing Object.}
We identify a failure mode of the head-expansion baseline model. The baseline fails to accurately predict the shape of private classes. We hypothesize that if a model consistently predicts the same object regardless of size variations, the model can accurately predict the shape of the object as well. To this end, we extend the domain mixing method Classmix~\cite{olsson2021classmix}, which selects half of the classes from the source and appends them to the target image to learn domain-invariant features. On top of the Classmix, we introduce an additional step where we select one more thing class from the source image, resize it, and paste it to the random location of a target image. The mixed target image contains the same objects as the source image, but the sizes of the objects are different. Therefore, the model learns not only domain-invariant representations but also size-invariant representations by learning from the mixed target images and the source images. It enables the model to better capture the shapes of both common and private class objects. This extension enhances the robustness of the model to size variations, contributing to the accurate prediction of the shape of unknown classes leading to superior open-set domain adaptation performance.

%The Resizing class process is as follows, we first resize the source image and label $x_s$,$y_s$ using downsample function $\zeta(\cdot,\cdot)$ by scale factor $s_r$
%\begin{align}
%x_s^r,y_s^r=\zeta(x_s,1/s_r),\zeta(y_s,1/s_r),
%\end{align}
%where $x_s^r$, and $y_s^r$ represent downsampled image and label.
%\begin{align}
%5x_t^{m}[b_1:b_1+H/s_r,b_2:b_2+H/s_R]=M_r \odot x_s^r + (1- M_r) \odot x_t^{m}[b_1:b_1+H/s_r,b_2:b_2+H/s_r],
%\end{align}
%where $b_1$, $b_2$ denote 

%To address this, we extend the use of the existing data augmentation method Classmix~\cite{olsson2021classmix} to learn size-robust features. Initially, Classmix~\cite{olsson2021classmix} selects half of the classes from the source and appends them to the target image. The model then learns from the mixed images, learning domain-robust features. In our adaptation, we introduce an additional step where we select one more thing class from the source, resize it, and paste it randomly to the target. When training the model, the newly generated mixed target and source images have different sizes but the same objects. We use joint training to make the same predictions. This extension enhances the robustness of the model to size variations, contributing to the accurate prediction of the shape of \emph{unknown}. 
%The pseudocode for the implementation of ClassMix~\cite{olsson2021classmix} with resizing is provided in Algorithm~\ref{al:classmix}, where the returned values \(x^{m}_t, \hat{y}^{m}_t\) are assigned to \eqref{eq:new_target_loss}.
\paragraph{Attaching Private.}
As described in Section 3.2, to address the challenge of learning target private classes, we extend the segmentation head. The extended head is trained with the target pseudo-labels which contain the private labels. However, since there are no private classes in the source image, we cannot utilize the source data to update the parameters of the additional head. To overcome this inefficiency in learning, we also copy target private class objects and paste them into a source image.

Given a target image, we create a target private mask consisting of 1 for private classes and 0 for common classes using the target pseudo-labels. With the target private mask, we copy the private regions in the target image to a source image, resulting in a private class-mixed source image. Similarly, by combining the labels of the source and the pseudo-labels of the target, we generate mixed source labels. This augmentation offers a significantly larger dataset for learning to reject private class objects, leading to improved open-set domain adaptation performance.

We formalize the attaching private process as follows. We use a target private mask \(M_{u}\) from Eq. \ref{eq:target_private}.
Based on \(M_{u}\), we generate a mixed source image $x_{s}^m$ and the corresponding source label \(y_{s}^m\) using the following equations:
\begin{align}
x_{s}^m = M_{u} \odot x_t + (1 - M_{u}) \odot x_s, \\
y_{s}^m = M_{u} \odot \hat{y}_{tp} + (1 - M_{u}) \odot y_s,
\end{align}
where $x^m_s$ and $y^m_s$ denote the mixed source image and the corresponding label. $x_t$ and $\hat{y}_{tp}$ denote the target image and its pseudo-label. The mixed image \(x_{s}^m\) and the mixed label \(y_{s}^m\) are applied to Eq. \eqref{eq:source_cleanloss}, instead of $x_s$ and $y_s$.
%  $x_{m}^t \leftarrow M \odot x^s + (1 - M) \odot x^t$ \tcp*{Mix target images.}
  
%  $\hat{y}_{m}^t \leftarrow M \odot y^s + (1 - M) \odot \hat{y}^t$ \tcp*{Mix target labels.}
%The pseudocode for the implementation of ClassMix~\cite{olsson2021classmix} with resizing is provided in Algorithm~\ref{al:bimix}, where the returned values \(x^{m}_s, \hat{y}^{m}_s\) are assigned to \eqref{eq:new_source_cleanloss}.

%\begin{algorithm}[H]
%\SetAlgoLined
%  \caption{ClassMix Algorithm}
%  \KwData{labeled source $x^s,y^s$ and unlabeled target $x^t$, teacher segmentation network $g_\theta$.}
%  \KwResult{Write here the expected result}
  
%  $SB \leftarrow g_\theta(x^t)$\;
  
%  $\hat{y^t} \leftarrow \text{argmax}_{c} SB(i, j, c)$\tcp{Take pixel-wise argmax over classes.}
  
%  $C \leftarrow$ Set of different classes present in $S\tilde{A}$\
  
%  $c \leftarrow$ Randomly selected subset of $C$ such that $|c| = |C|/2$\;
  
%  $c_r \leftarrow$ Randomly selected one thing class of $C$ but not in $c$\;
  
%  \For{all $i, j$}{
%    $M(i, j) =
%    \begin{cases}
%      1, & \text{if } S\tilde{A}(i, j) \in c \\
%      0, & \text{otherwise}
%    \end{cases}$ \tcp*{Create binary mask.}
%  }
  
%  $x_{m}^t \leftarrow M \odot x^s + (1 - M) \odot x^t$ \tcp*{Mix target images.}
  
%  $\hat{y}_{m}^t \leftarrow M \odot y^s + (1 - M) \odot \hat{y}^t$ \tcp*{Mix target labels.}
%  \Return{\(x_{m}^t, \hat{y}_{m}^t\)}\;
%\end{algorithm}


==> sec/5_result.tex <==
\input{sec/table/main1}
\input{sec/table/main2}
\section{Experiments}
\label{sec:results}

\input{sec/figure/qualitative_result}
\input{sec/figure/qualitative_result2}


\subsection{Experimental Setup}
\paragraph{Datasets.}
% Describe datasets used, statistics (# images, train/val/test splits)
We evaluated our framework over two challenging synthetic-to-real scenarios in autonomous driving, i.e., GTA5$\rightarrow$Cityscapes and SYNTHIA$\rightarrow$Cityscapes. GTA5 \cite{richter2016playing} is a synthesized dataset, which consists of 24,966 images with a resolution of 1914x1052. For SYNTHIA \cite{ros2016synthia}, it is also a synthesized dataset, which contains 9,400 images with resolution $1280 \times 760$. CityScapes \cite{cordts2016cityscapes} is a real-image dataset with 2,975 training samples and 500 validation samples with resolution $2048 \times 1024$. It shares the common 19 classes with GTA and 16 classes with SYNTHIA.
\paragraph{Scenario Construction.}
Using these datasets, we established new scenarios tailored for the OSDA-SS task. First, to create new classes emerging in the target domain that are not present in the source domain, we selected certain source classes to be removed. In autonomous driving scenarios, the classes that are likely to emerge in the target domain are expected to be ``thing" classes. Stuff classes representing the background area typically do not emerge as new classes. Therefore, we selected specific classes from the ``thing" categories to be excluded. The following list denotes the classes designated as unknown class in GTA5 and SYNTHIA. 
\begin{itemize}
\item GTA5: ``pole", ``traffic sign", ``person", ``rider", ``truck", and ``train". \\
\item SYNTHIA: ``pole", ``traffic sign", ``person", ``rider", ``truck", ``train", and ``terrain".
\end{itemize}
Notably, SYNTHIA includes the ``terrain", which inherently lacks labels from the outset.
Second, to prevent the selected classes from being trained in the source domain, pixels corresponding to those classes were treated as ``ignore" and were not incorporated into the loss function during training.
Finally, during the evaluation of the target domain, 
the classes listed above were treated as a single unknown class.
\paragraph{Evaluation Metrics.}
Previous works \cite{hoyer2022daformer,melas2021pixmatch,hoyer2022hrda,hoyer2023mic} used mIoU (mean Intersection-over-Union) as the evaluation metric, which averaged the IoU of each class. Since we treated unknown classes as a single unknown class, simply averaging would diminish the impact of private classes significantly. Therefore, inspired by \cite{fu2020learning}, we utilized the harmonic mean of the mean IoU score for known classes (common) and the IoU score for one unknown class (private) as our evaluation metric, known as the H-Score.

\paragraph{Implementation Details.} 
We adopted DAFormer~\cite{hoyer2022daformer} network with the MiT-B5 encoder~\cite{xie2021segformer} pre-trained on imageNet-1K~\cite{deng2009imagenet}. We followed the multi-resolution self-training strategy and training parameters of MIC~\cite{hoyer2023mic}. The network was trained with AdamW~\cite{loshchilov2017decoupled}. The learning rates were set to 6e-5 for the backbone and 6e-4 for the decoder head, with a weight decay of 0.01 and linear learning rate warm-up over 1.5k steps. EMA factor was \(\alpha\)=0.999. Additionally, we utilized the Rare Class Sampling~\cite{hoyer2022daformer}, ImageNet Feature Distance~\cite{hoyer2022daformer}, DACS~\cite{tranheden2021dacs} data augmentation, and Masked Image Consistency module~\cite{hoyer2023mic}. We trained on a batch of two $512 \times 512$ random crops for 40k iterations.

% Questions to be addressed:
% - What are the values of parameter X?
% - How did you select this particular value? e.g., cross-validation with grid search

\paragraph{Baselines.} 
% Comparison to the state-of-the-art
We compared our approach with two scenarios. The first scenario comprised the Open-Set Domain Adaptation (OSDA) method, specifically OSBP~\cite{saito2018open}, and Universal Domain Adaptation (UniDA) methods like UAN~\cite{you2019universal} and UniOT~\cite{jang2022unknown}, which were capable of rejecting unknowns but were primarily designed for classification tasks. 
The second scenario was Unsupervised Domain Adaptation (UDA) methods incapable of rejecting unknown classes, which included AdaptSegNet~\cite{tsai2018learning}, Pixmatch~\cite{melas2021pixmatch}, DAFormer~\cite{hoyer2022daformer}, HRDA~\cite{hoyer2022hrda}, and MIC~\cite{hoyer2023mic}. 
In the UDA method, we assigned the unknown label during inference for regions with low confidence scores. For OSDA and UniDA methods, we replaced the classification network with a segmentation network with DeepLabv2~\cite{chen2017deeplab} using ResNet-101~\cite{he2016deep} as the backbone, and adopted the image-level methods to operate at the pixel-level.

% \begin{table}[t]
% \resizebox{\columnwidth}{!}{%
% \setlength{\tabcolsep}{1.5pt}
% \renewcommand{\arraystretch}{1.4}
% \begin{tabular}{c|ccccc}
% \specialrule{1.5pt}{0.1pt}{1pt}
% \multirow{2}{*}{Method} & \multicolumn{5}{c}{GTA5 $\rightarrow$ Cityscapes} \\
                        % & Common     &      & Private    &     & H-Score    \\ \hline
% \rowcolor[gray]{.9} BUS (Ours)              & \textbf{72.33}      &      & \textbf{53.95}      &     & \textbf{61.81}      \\ \hdashline
% w/o resizing            & 70.79      &      & 46.34      &     & 56.01      \\
% w/o attach private      & 66.85      &      & 34.29      &     & 45.89     \\
% \specialrule{1.5pt}{0.1pt}{1pt}
% \end{tabular}%
% }
% \end{table}

\subsection{Comparisons with the State-of-the-Art}
Table~\ref{tab:table-name1} showed the experimental results for GTA5 $\rightarrow$ Cityscapes and SYNTHIA$\rightarrow$ Cityscapes, respectively. The classification methods struggled to accurately discriminate the private class in semantic segmentation tasks, which demanded a higher degree of spatial information. The UDA methods also faced challenges in effectively distinguishing private class leveraging a confidence-based approach.
In contrast, our proposed approach significantly outperformed the other comparison methods based on the H-Score. Especially, compared to the best baseline DAF \cite{hoyer2022daformer}, our method, BUS, achieved a performance improvement of about $+38.45\%$ in GTA $\rightarrow$ Cityscapes and about $+25.92\%$ in SYNTHIA $\rightarrow$ Cityscapes. This experiment demonstrated the effectiveness of our method in discriminating private classes while maintaining classification performance for common classes.

A more detailed examination revealed that we achieved a significant improvement in the private class IoU score to approximately $+39.32\%$ compared to the DAF \cite{hoyer2022daformer}, and also an increase in the common class mIoU score of about $+8.51\%$ compared to the HRDA \cite{hoyer2022hrda}. This showed that our proposed method not only improved the performance of the private class but also contributed to a slight improvement in the common classes.


\begin{table}[t]
    \setlength{\tabcolsep}{2.2pt}
    \renewcommand{\arraystretch}{1.6}
    \resizebox{\columnwidth}{!}{
    % \begin{tabular}{cccc|ccc}
    \begin{NiceTabular}{cccc|ccc}
        \specialrule{2.pt}{1pt}{1pt}
        \multicolumn{4}{c|}{Method}                                     & \multicolumn{3}{c}{GTA5 $\rightarrow$  Cityscapes} \\ \hline
        \multicolumn{1}{c|}{Config.} & \# Head      & DECON & OpenReMix & Common     & Private     & H-Score    \\ \hline
        \multicolumn{1}{c|}{A}       & \textit{C}   &       &           & 58.17      & 11.87       & 19.71      \\
        \multicolumn{1}{c|}{B}       & \textit{C}+1 &       &           & 70.37      & 31.78       & 43.79      \\ \dashedline
        \multicolumn{1}{c|}{C}       & \textit{C}+1 &  \multicolumn{1}{c}{\checkmark}     &           & 71.16      & 48.34       & 57.57      \\
        \multicolumn{1}{c|}{D}       & \textit{C}+1 &       &    \multicolumn{1}{c}{\checkmark}       & 71.52      & 49.26       & 58.34      \\
        \rowcolor[gray]{.9} \multicolumn{1}{c|}{\textbf{Ours}}    & \textit{C}+1 &   \multicolumn{1}{c}{\checkmark}    &    \multicolumn{1}{c}{\checkmark}       & \textbf{72.33}      & \textbf{53.95}       & \textbf{61.81}  \\
        \specialrule{2.pt}{0.1pt}{1pt}
    \end{NiceTabular}%
    }
    \vspace{-2mm}
    \caption{Ablation study of the components in our BUS framework. Configuration A, B, C, and D represent confidence-based MIC, head-expansion, DECON, and OpenReMix, respectively.}
    \label{tab:ablation1}
    \vspace{-4mm}
\end{table}

%qualtative2



\subsection{Qualitative Evaluation}
% To validate the performance of our method, we conducted further qualitative evaluation to assess a segmentation performance with baselines.
% We show Figure.~\ref{fig:qu1} visualize map on the GTA5 $\rightarrow$  Cityscapes. Compared to the baseline model and it
To validate the performance of our method, we conducted additional qualitative evaluations to assess segmentation performance against baselines. We compared our method with MIC, confidence-based MIC (Config. A), and the head-expansion approach (Config. B) in the GTA $\rightarrow$ Cityscapes (see Figure~\ref{fig:qu1}). Furthermore, we compared our method with the head-expansion approach (Config. B), the incorporation of a new DECON loss (Config. C), and the utilization of the new OpenReMix (Config. D) in the SYNTHIA $\rightarrow$ Cityscapes(see Figure~\ref{fig:qu2}).
In Figure~\ref{fig:qu1}, we observe that the UDA method MIC struggles with private class classification in OSDA-SS, designed for UDA without considering unknown classes. Even baselines like confidence-based MIC (Config. A) and head-expansion (Config. B) face challenges in private class classification. Although head-expansion shows promise, it has limitations in classifying specific pixels in private classes. In contrast, our method excels, particularly in discerning object size.
In Figure~\ref{fig:qu2}, our DECON loss and OpenReMix yield outstanding classification performance. These novel components, a contrastive loss and domain mixing augmentation, respectively, greatly enhance classification. BUS, our proposed method, demonstrates remarkable classification quality. Notably, even without private class information, it effectively classifies unknown classes using DECON loss and OpenReMix.
% Furthermore, we observed that our proposed method DECON loss and OpenReMix showed outstanding classification performance in Figure~\ref{fig:qu2}. DECON loss which a new designed contrastive loss and OpenRemix which is a novel domain mixing augmentation reveals that each proposed components highly help enhancing classification performance, respectively. At this end, the proposed method, BUS, demonstrated its remarkable classification quality. Despite the absence of private class information, our proposed ethod is able to classify the unknown classes through the proposed DECON loss and OpenReMix.

% As shown in Figure~\ref{fig:qu1}, we found that the UDA method MIC struggles to classify private classes in the OSDA-SS scenario, as it was originally designed for UDA and does not consider the presence of unknown classes. Even reasonable baselines such as confidence-based MIC (Config. A) and head-expansion approach (Config. B) encountered challenges in classifying private classes. While head-expansion appeared promising, it demonstrated limitations in classifying certain pixels within private classes. In contrast to previous approaches, our proposed method demonstrates notable classification performance, particularly in discerning whether the object is large or small.

\subsection{Ablation Study}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
%\begin{table}[]
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{l|ccccc}
%\specialrule{1.5pt}{1pt}{1pt}
%\multirow{2}{*}{Method} & \multicolumn{5}{c}{GTA5 $\rightarrow$ Cityscapes} \\ \cline{2-6}
%                        & Common     &      & Private    &     & H-Score    \\ \hline
%BUS (Ours)              & 72.33      &      & 53.95      &     & 61.81      \\ \cdashedline
%w/o resizing            & 70.79      &      & 46.34      &     & 56.01      \\
%w/o attach private      & 66.85      &      & 34.29      &     & 45.89     \\
%\specialrule{1.5pt}{1pt}{1pt}
%\end{tabular}%
%}
%\end{table}

% ===================================================================================

% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \setlength{\tabcolsep}{2.pt}
% \renewcommand{\arraystretch}{1.8}
% \begin{tabular}{cccc|ccc}
% \specialrule{1.5pt}{1pt}{1pt}
% \multicolumn{4}{c|}{Method}                                     & \multicolumn{3}{c}{GTA5 $\rightarrow$  Cityscapes} \\ \hline
% \multicolumn{1}{c|}{Config.} & \# Head      & DECON & OpenReMix & Common     & Private     & H-Score    \\ \hline
% \multicolumn{1}{c|}{A}       & \textit{C}   &       &           & 71.15      & 26.67       & 38.80      \\
% \multicolumn{1}{c|}{B}       & \textit{C}+1 &       &           & 70.37      & 31.78       & 43.79      \\ \hdashline
% \multicolumn{1}{c|}{C}       & \textit{C}+1 &  \checkmark     &           & 71.16      & 48.34       & 57.57      \\
% \multicolumn{1}{c|}{D}       & \textit{C}+1 &       &    \checkmark       & 71.52      & 49.26       & 58.34      \\
% \rowcolor[gray]{.9} \multicolumn{1}{c|}{Ours}    & \textit{C}+1 &   \checkmark    &    \checkmark       & 72.33      & 53.95       & 61.81  \\
% \specialrule{1.5pt}{1pt}{1pt}
% \end{tabular}%
% }
% \caption{\label{tab:ablation1} Ablation of the components of the BUS framework.}
% \end{table}

%\input{sec/figure/qualitative_result2}

% [GMPARK] Experiment 쓸때는 반드시 과거시제를 쓰세요.
\paragraph{Ablation Study.}
We conducted an ablation study for the proposed components of the BUS framework on GTA5 $\rightarrow$ Cityscapes. In Table~\ref{tab:ablation1}, row A and B represent the confidence-based threshold and head-expansion, respectively. We used the confidence-based threshold and head-expansion as baselines for our ablation study. As shown in Table~\ref{tab:ablation1}, the confidence-based threshold (config.A) recorded inferior performance to the head-expansion (config.B). It reveals that leveraging the head-expansion is effective in detecting unknown classes. 
% baselines that reasonably extended existing UDA methods, MIC. row A represents the confidence-based threshold an head-expansion, respectively. 
achieving H-Scores of 19.71 and 43.79. When combined with DECON on head-expansion, we gained an H-Score of 13.78 (Table \ref{tab:ablation1}, row c). we also study about effect of OpenReMix. we gained 14.55 from OpenReMix.
Lastly, Ours, using both DECON and OpenReMix on head-expansion, achieved a significantly improved H-Score of 18.02. Figure ~\ref{fig:qu1} shows a clear improvement in predicting the unknown compared to Figure ~\ref{fig:qu1} (b), and we can observe synergy in overcoming individual drawbacks when compared to Figure ~\ref{fig:qu1} (c) and Figure ~\ref{fig:qu1} (d).

%T.C only using the DECON on Config. B gained an H-Score of 13.78. Config.D only using OpenReMix on Config. B improved the H-Score to 14.55. In Figure 4, it was evident that Config.D captured the shape of unknown better compared to Config.B. Lastly, Ours, using both DECON and OpenReMix on Config.B, achieved a significantly improved H-Score of 18.02. Figure 4 showed a clear improvement in predicting unknown compared to B, and synergy was observed in overcoming individual drawbacks when compared to Config. C and Config.D. Figure ~\ref{fig:qu1} shows the qualitative result of each rows. 
%\paragraph{Dilation Mask.}
%window size, number of windows
%\paragraph{ClassMix with Resize.}
%size, number of classes

% \input{sec/figure/qualitative_result2}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\vspace{0.3mm}
\resizebox{\columnwidth}{!}{%
\setlength{\tabcolsep}{10.pt}
\renewcommand{\arraystretch}{1.2}
\begin{NiceTabular}{c|c|c|c}
\specialrule{1.5pt}{0.1pt}{1pt}
% \hline
\multicolumn{4}{c}{GTA5 $\rightarrow$ Cityscapes}           \\ \hline
\multicolumn{1}{c}{\# of Unknown} \vline & Config. A & Config. B & Ours  \\ \hline
\multicolumn{1}{c}{6}       \vline      & 19.71          & 43.79              & \multicolumn{1}{c}{61.81} \\
\multicolumn{1}{c}{4}       \vline      & 11.73          & 41.54              & \multicolumn{1}{c}{52.17} \\
\multicolumn{1}{c}{2}       \vline      & 9.43           & 41.51              & \multicolumn{1}{c}{56.73} \\

\specialrule{1.5pt}{0.2pt}{1pt}
% \bottomrule
\end{NiceTabular}%
}
\vspace{-3mm}
\caption{\label{tab:numof_unknown} The comparison of the number of unknown classes. Config.A denotes confidence-based MIC and config.B denotes head-expansion.}
\vspace{-5mm}
%  Unknown 갯수에 따른 실험
\end{table}
\paragraph{Unknown Proportion.}
We conducted experiments varying the number of unknown classes. When the number of unknown classes was 6, 4, and 2, we compared two MIC baselines with Ours. For the case with 4 unknown classes, we selected (``pole", ``traffic sign", ``person", ``rider"), and for 2 unknown classes, we chose (``person", ``rider"). Table ~\ref{tab:numof_unknown} shows that Ours consistently outperforms the baselines, regardless of the change in the number of unknown classes.
%\paragraph{Influence of threshold.}
%\paragraph{Influence of SAM ratio.}

==> sec/6_conclusion.tex <==
\section{Conclusion}
   \label{sec:conclusions}
To tackle this challenging task, we proposed a novel OSDA method named BUS. Our approach includes DECON, a new dilation-erosion-based contrastive loss designed to rectify less confident and erroneous predictions near class boundaries. In addition, we proposed OpenReMix, a technique guiding the model to acquire size-invariant features and efficiently train the expanded head by mixing unknown objects from the target into the source. OpenReMix encouraged our model to concentrate on the shape information of unknown entities. Through extensive experiments, we demonstrated the efficacy of our proposed method on public benchmark datasets, surpassing existing approaches by a significant margin. We anticipate that our work will be widely applied in research or the industry field, providing a strong baseline to detect unexpected, unseen objects in mission-critical scenarios.

==> sec/figure/fig_main.tex <==


\begin{figure*}[t] %%% t: top, b: bottom, h: here

% \begin{center}
\centering
\includegraphics[width=1\textwidth]{sec/figure/main_figure_3.pdf}
\vspace{-6mm}
% \end{center}

\caption{Overview of our proposed Boundary and Unknown Shape-Aware (BUS) method. 
We generate the mixed source image $\text{Img}_{M_{s}}$ and the mixed target image $\text{Img}_{M_{t}}$ from OpenReMix. The model is trained using the mixed source label and the mixed target pseudo-labels with supervised loss and adaptation loss, respectively. Especially, the expanded head is trained with the parts that predicted as unknown in pseudo-labels. Pseudo-labels are generated by thresholding the softmax probability and passing through the refinement network. DECON loss utilizes the dilation and erosion operations to distinguish the known and unknown classes near the boundaries.
\vspace{-3mm}}
\vspace{-3mm}
\label{fig:long}

\label{fig:onecol}

\end{figure*}

%\begin{figure*}
%   \centering
%   \begin{subfigure}{1\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{1\linewidth}{0pt}}
%     \caption{main figure.}
%     \label{fig:short-a}
%   \end{subfigure}
% \end{figure*}

==> sec/figure/motivation1.tex <==

\begin{figure}[t] %%% t: top, b: bottom, h: here
\includegraphics[width=\columnwidth]{sec/figure/motivation_fig1.png}
\caption{Motivation Figure}
\label{fig:longa}
\end{figure}

==> sec/figure/qualitative_result.tex <==

\begin{figure*}[t] %%% t: top, b: bottom, h: here

\centering

\includegraphics[width=1\textwidth]{sec/figure/qualitative_figure1_update.jpg}
\vspace{-8mm}
\caption{Qualitative comparison of our method with MIC, confidence-based MIC (config.~A), and head-expansion (config.~B) on the GTA5 $\rightarrow$ Cityscapes. GT represents ground truth.}

\label{fig:qu1}

\label{fig:onecol}

\end{figure*}


==> sec/figure/qualitative_result2.tex <==
\begin{figure*}[t] %%% t: top, b: bottom, h: here

\centering

\includegraphics[width=1\textwidth]{sec/figure/qualitative_figure2_update.jpg}
\vspace{-8mm}
\caption{Qualitative comparison of our method with head-expansion (config.~B), DECON (config.~C), and OpenReMix (config.~D) on the SYNTHIA $\rightarrow$ Cityscapes. GT represents ground truth.}
% \caption{Qualitative results of our method on the SYNTHIA $\rightarrow$ Cityscapes scenario. Config.~A denotes confidence-based MIC and config.~B denotes head-expansion.}
\vspace{-4mm}
\label{fig:qu2}

\label{fig:onecol}

\end{figure*}

==> sec/intro_copy.tex <==
\section{Introduction}
\label{sec:intro}


%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/table/ablation1.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc|ccc}
\multicolumn{4}{c|}{Method}                                     & \multicolumn{3}{c}{GTA5 $\rightarrow$  Cityscapes} \\ \hline
\multicolumn{1}{c|}{Config.} & \# Head      & DECON & OpenReMix & Common     & Private     & H-Score    \\ \hline
\multicolumn{1}{c|}{A}       & \textit{C}   &       &           & 71.15      & 26.67       & 38.80      \\
\multicolumn{1}{c|}{B}       & \textit{C+1} &       &           & 70.37      & 31.78       & 43.79      \\ \hline
\multicolumn{1}{c|}{C}       & \textit{C+1} &       &           & 71.16      & 48.34       & 57.57      \\
\multicolumn{1}{c|}{D}       & \textit{C+1} &       &           & 71.52      & 49.26       & 58.34      \\
\multicolumn{1}{c|}{Ours}    & \textit{C+1} &       &           & 72.33      & 53.95       & 61.81      \\ \hline
\end{tabular}%
}
\end{table}

==> sec/table/table.tex <==


\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{Cityscapes $\rightarrow$ IDD} & \multicolumn{3}{c}{Cityscapes $\rightarrow$ SYNTHIA} \\ \cline{2-7} 
                        & Common      & Private      & H-Score     & Common    & Private    & H-Score    \\ \hline
BUDA                    & 37.3        & 18.5         & 24.7         & 36.2        & 17.0         & 23.1        \\
MIC                     &   54.3        &    24.1      &    34.4       & 61.80        & 1.8       & 3.5       \\
\textbf{BUS}            & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}         & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}        \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
%\caption{\label{tab:BUDA_experiment} Comparison of BUS with BUDA on private classes 'auto rickshaw' and 'animal'.}
\caption{\label{tab:BUDA_experiment} Additional experiments on CS $\rightarrow$ IDD.}%Comparison of BUS with BUDA.}
\vspace{-4mm}
\end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
Method & Common & Private & H-Score \\ \hline
MIC    & 60.35 \(\pm\) 6.55 & 61.38 \(\pm\) 10.61   & 59.66 \(\pm\) 11.13   \\
\textbf{BUS}    & \textbf{64.16 \(\pm\) 7.07}  & \textbf{66.22 \(\pm\) 11.77}   & \textbf{64.33 \(\pm\) 3.45}   \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
\caption{\label{tab:random_private} H-Score on randomly selecting unseen classes.}
\vspace{-3mm}
\end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{SYNTHIA $\rightarrow$ Cityscapes} & \multicolumn{3}{c}{Cityscapes $\rightarrow$ IDD} \\ \cline{2-7} 
                        & Common      & Private      & H-Score     & Common    & Private    & H-Score    \\ \hline
BUDA                    & 36.2        & 17.0         & 23.1         & 37.3        & 18.5       & 24.7        \\
MIC                     & 61.80          & 1.8         & 3.5         & 54.3        & 24.1       & 34.4        \\
\textbf{BUS}                    & 0.0          & 0.0         & 0.0         & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}        \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
%\caption{\label{tab:BUDA_experiment} Comparison of BUS with BUDA on private classes 'auto rickshaw' and 'animal'.}
\caption{\label{tab:BUDA_experiment} Additional experiments on CS $\rightarrow$ IDD.}%Comparison of BUS with BUDA.}
\vspace{-4mm}
\end{table}

==> sec_final/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec_final/figure/OpenReMix.tex <==
\begin{figure}[t] %%% t: top, b: bottom, h: here

\centering

\includegraphics[width=\columnwidth]{sec_final/figure/OpenRemix.png}
\vspace{-8mm}
\caption{Example of OpenReMix: the source image is mixed with a private class from the target image (red mask). The target image is mixed by Classmix~\cite{olsson2021classmix} (green mask) and is additionally mixed with the resized thing class from the source image (yellow mask).
}

\label{fig:OpenReMix}

\end{figure}

==> sec_final/table/ablation1.tex <==
\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccc|ccc}
\multicolumn{4}{c|}{Method}                                     & \multicolumn{3}{c}{GTA5 $\rightarrow$  Cityscapes} \\ \hline
\multicolumn{1}{c|}{Config.} & \# Head      & DECON & OpenReMix & Common     & Private     & H-Score    \\ \hline
\multicolumn{1}{c|}{A}       & \textit{C}   &       &           & 71.15      & 26.67       & 38.80      \\
\multicolumn{1}{c|}{B}       & \textit{C+1} &       &           & 70.37      & 31.78       & 43.79      \\ \hline
\multicolumn{1}{c|}{C}       & \textit{C+1} &       &           & 71.16      & 48.34       & 57.57      \\
\multicolumn{1}{c|}{D}       & \textit{C+1} &       &           & 71.52      & 49.26       & 58.34      \\
\multicolumn{1}{c|}{Ours}    & \textit{C+1} &       &           & 72.33      & 53.95       & 61.81      \\ \hline
\end{tabular}%
}
\end{table}

==> sec_final/table/main1.tex <==
% \usepackage{colortbl}
% \begin{tabular}{|>{\columncolor[gray]{0.8}}c|c|c|c|c|c|c|c|}

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{2.pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lccccccccccccc>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c}
\specialrule{1.5pt}{1pt}{0pt}
% \toprule
\multicolumn{1}{c|}{Method}                                   & Road  & S.walk & Build. & Wall  & Fence & Light & Veget. & Terrain & Sky   & Car   & Bus   & M.bike & \multicolumn{1}{c|}{Bike}  & Common & Private & H-Score \\ \hline
\multicolumn{17}{c}{\textbf{GTA5 $\rightarrow$ Cityscapes}}                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{l|}{OSBP ~\cite{saito2018open}}    & 4.92 & 3.93  & 42.8  & 2.55 & 6.04 & 14.29 & 68.58  & 26.50   & 44.21 & 41.78 & 0.94 & 7.20  & \multicolumn{1}{c|}{3.42} &  20.55  &  4.49   &  7.34   \\
\multicolumn{1}{l|}{UAN ~\cite{you2019universal}}     & 65.97 & 23.41  & 76.41 & 37.26 & 18.50 & 20.13  & 80.57   & 30.37 & 82.47 & 77.35  & 27.80 & 16.62 & \multicolumn{1}{c|}{0.00}  &  38.00  &  3.59    &  6.56     \\
\multicolumn{1}{l|}{UniOT ~\cite{jang2022unknown}} & 17.67  & 5.14   & 44.86   & 55.45  & 2.31  & 52.61  & 40.01   & 3.37    & 79.43  & 52.87  & 52.31  & 7.18   & \multicolumn{1}{c|}{0.00}  &  20.20  &  5.36    &  7.49    \\ \hline
\multicolumn{1}{l|}{ASN~\cite{tsai2018learning}}          & 82.34 & 2.21   & 75.30   & 8.01  & 3.52  & 9.99  & 71.96  & 15.61   & 70.97 & 77.16 & 22.59 & 20.8   & \multicolumn{1}{c|}{0.06}  &  35.43  &  10.84   &  16.60   \\
\multicolumn{1}{l|}{Pixmatch ~\cite{melas2021pixmatch}}            & 79.27 & 2.06   & 72.36  & 6.96  & 2.94  & 11.07 & 76.29  & 23.23   & 77.72 & 79.77 & 44.72 & 18.02  & \multicolumn{1}{c|}{0.01}  &  38.03  &  9.46    &  15.15   \\
\multicolumn{1}{l|}{DAF~\cite{hoyer2022daformer}}            & 94.26 & 48.69  & 83.47  & 38.67 & 32.83 & 41.71 & 87.79  & 39.15   & \textbf{93.59} & 85.29 & 47.04 & 28.36  & \multicolumn{1}{c|}{46.86} &  61.26  &  14.63   &  23.36   \\
\multicolumn{1}{l|}{HRDA ~\cite{hoyer2022hrda}}                & 95.14 & 62.58  & 82.92  & 47.44 & 43.57 & 53.18 & 88.26  & 44.42   & 92.92 & 90.23 & 57.43 & 14.71  & \multicolumn{1}{c|}{56.83} &  63.82  &  12.13   &  20.39   \\
\multicolumn{1}{l|}{MIC ~\cite{hoyer2023mic}}                 & 93.26 & 58.96 & 79.30  & 21.62 & 31.41 & 39.32 & 85.48  & 31.94   & 91.64 & 88.16 & 44.77 & 47.64  & \multicolumn{1}{c|}{42.77} &  58.17  &  11.87   &  19.71   \\ \hline
\multicolumn{1}{l|}{BUS \textbf{(Ours)}}                & \textbf{95.19} & \textbf{66.36}  & \textbf{90.36}  & \textbf{57.20} & \textbf{56.17} & \textbf{56.68} & \textbf{91.07}  & \textbf{49.46}   & 93.29 & \textbf{93.55} & \textbf{64.79} & \textbf{58.03}  & \multicolumn{1}{c|}{\textbf{68.21}} &  \textbf{72.33}  &  \textbf{53.95}   &  \textbf{61.81}   \\
\specialrule{1.5pt}{1pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
% \caption{\label{tab:table-name1} Semantic segmentation performance on OSDA-SS. ASN denotes AdapSegNet~\cite{tsai2018learning} and DAF denotes DAFormer~\cite{hoyer2022daformer}.}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{2.pt}
\renewcommand{\arraystretch}{1.}
% \col
\begin{tabular}{ccccccccccccc>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c>{\columncolor[gray]{0.9}}c}
% \hline
\specialrule{1.5pt}{1pt}{1pt}
\multicolumn{1}{c|}{Method}                  & Road  & S.walk & Build. & Wall  & Fence & Light & Veget. & Sky   & Car   & Bus   & M.bike & \multicolumn{1}{c|}{Bike}  & Common                                            & Private                                          & H-Score                                          \\ \hline
\multicolumn{16}{c}{\textbf{SYNTHIA $\rightarrow$ Cityscapes}}                                                                                                                                                                                                                                                                  \\ \hline
\multicolumn{1}{l|}{OSBP~\cite{saito2018open}}       &    6.71   &    9.49    &   49.83     &   0.70    &  0.0     &   0.76    &   26.03     &   36.91    &   20.04    &   4.76    &   2.90     & \multicolumn{1}{c|}{8.70}      &                  13.20                                 &         4.90                                         &           7.14                                       \\
\multicolumn{1}{l|}{UAN~\cite{you2019universal}}  &   33.24    &   19.03    &    71.49    &    4.02    &   0.05    &   14.34    &    75.78   &    81.06    &   53.88    &   19.34    &   8.14    &    \multicolumn{1}{c|}{21.84}      & 31.30 & 4.53 & 7.91 \\
\multicolumn{1}{l|}{UniOT~\cite{jang2022unknown}}      &  0.00     &   16.79     &  18.52      &  1.05     &  6.49     &  16.8     &  14.52      &   57.4    &  6.48     &   2.59    &   3.73     & \multicolumn{1}{c|}{3.88}     & 12.35 & 5.49 & 7.06 \\ \hline
\multicolumn{1}{l|}{ASN~\cite{tsai2018learning}} &   77.31    &    15.14    &    78.59    &    1.29   &   0.07    &   14.82    &    69.7    &    82.86   &    63.06   &    30.2   &    5.16   & \multicolumn{1}{c|}{20.76}      &      35.30                                             &  5.36                                                &9.31                                                  \\
\multicolumn{1}{l|}{Pixmatch~\cite{melas2021pixmatch}}   & 74.16      & 8.15       & 76.21       & 0.01      & 0.0      & 5.64      & 44.15       & 63.76      & 44.66      & 17.27      & 0.13       & \multicolumn{1}{c|}{0.38}      & 26.30                                                  & 6.87                                                 & 11.00                                                 \\
\multicolumn{1}{l|}{DAF~\cite{hoyer2022daformer}}  & 70.10 & 39.65  & 83.09  & 22.75 & 4.66  & 41.19 & 81.56  & 91.79 & 84.36 & 51.13 & 43.78  & \multicolumn{1}{c|}{46.20} & 51.49                                             & 9.07                                             & 15.57                                            \\
\multicolumn{1}{l|}{HRDA~\cite{hoyer2022hrda}}       & 85.62 & 41.74  & 83.29  & 36.35 & 0.86  & 35.17 & 83.98  & 90.90 & 84.74 & 50.42 & 46.78  & \multicolumn{1}{c|}{58.33} & 54.68                                             & 12.68                                            & 20.82                                            \\
\multicolumn{1}{l|}{MIC~\cite{hoyer2023mic}}        & \textbf{88.31} & \textbf{70.71}  & 85.00  & 26.23 & \textbf{6.60}  & 35.27 & 84.80  & 91.41 & 81.47 & 53.62 & 55.39  & \multicolumn{1}{c|}{58.20} & 57.46                                             & 10.02                                            & 17.23                                            \\ \hline
\multicolumn{1}{l|}{BUS \textbf{(Ours)}}       & 87.57 & 49.05  & \textbf{88.05}  & \textbf{41.61} & 5.42  & \textbf{57.83} & \textbf{86.12}  & \textbf{92.13} & \textbf{88.43} & \textbf{60.92} & \textbf{59.83}  & \multicolumn{1}{c|}{\textbf{60.44}} & \textbf{62.15}                                             & \textbf{30.51}                                            & \textbf{41.49}                                            \\
\specialrule{1.5pt}{1pt}{1pt}
\end{tabular}%
}
\vspace{-2mm}
\caption{\label{tab:table-name1} Semantic segmentation performance on two different OSDA-SS benchmarks. ASN denotes AdapSegNet~\cite{tsai2018learning} and DAF denotes DAFormer~\cite{hoyer2022daformer}. Our method, BUS, outperformed state-of-the-art UDA methods, achieving a remarkable $+38.34\%$ H-score against DAFormer in GTA $\rightarrow$ Cityscapes and approximately $+20.67\%$ against HRDA in SYNTHIA $\rightarrow$ Cityscapes.}
\vspace{-3mm}
\end{table*}

% \begin{table*}[]
% \vspace{5mm}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllllllllllllll}
% \multicolumn{1}{l|}{Method}                 & \multicolumn{1}{c}{Road} & \multicolumn{1}{c}{S.walk} & \multicolumn{1}{c}{Build.} & \multicolumn{1}{c}{Wall} & \multicolumn{1}{c}{Fence} & sign & \multicolumn{1}{c}{Light} & \multicolumn{1}{c}{Veget.} & \multicolumn{1}{c}{Sky} & \multicolumn{1}{c}{Person} & rider & \multicolumn{1}{c}{Car} & \multicolumn{1}{c}{Bus} & \multicolumn{1}{c}{M.bike} & \multicolumn{1}{c|}{Bike} & \multicolumn{1}{c}{Common} & \multicolumn{1}{c}{Private} & \multicolumn{1}{c}{H-score} \\ \hline
% \multicolumn{19}{c}{SYNTHIA \(\xleftarrow{}\) CityScpaes}  \\ \hline
% \multicolumn{1}{l|}{OSBP (ECCV 2018)}       &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{UAN (CVPR 2021)}        &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{UniOT (NeuIPS 2022)}    &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \multicolumn{1}{l|}{AdapSegNet (CVPR 2018)} &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{Pixmatch (CVPR2021)}    &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{DAFormer (CVPR 2022)}   & 70.10                         & 39.65                           & 83.09                           & 22.75                         & 4.66                          & 41.19     & 81.56                          & 91.79                           & 84.36                        & 51.13                           & 43.78      & 46.2                        & 9.07                        &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{HRDA (ECCV 2022)}       &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{MIC (CVPR 2023)}        &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \multicolumn{1}{l|}{\textbf{Ours}}          &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \end{tabular}
% }
% \vspace{-3mm}
% \caption{\label{tab:table-name}main2.}
% \end{table*}

==> sec_final/table/main2.tex <==
% \begin{table*}[]
% \caption{\label{tab:table-name}main2.}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lllllllllllllllllll}
% \multicolumn{1}{l|}{Method}                 & \multicolumn{1}{c}{Road} & \multicolumn{1}{c}{S.walk} & \multicolumn{1}{c}{Build.} & \multicolumn{1}{c}{Wall} & \multicolumn{1}{c}{Fence} & sign & \multicolumn{1}{c}{Light} & \multicolumn{1}{c}{Veget.} & \multicolumn{1}{c}{Sky} & \multicolumn{1}{c}{Person} & rider & \multicolumn{1}{c}{Car} & \multicolumn{1}{c}{Bus} & \multicolumn{1}{c}{M.bike} & \multicolumn{1}{c|}{Bike} & \multicolumn{1}{c}{Common} & \multicolumn{1}{c}{Private} & \multicolumn{1}{c}{H-score} \\ \hline
% \multicolumn{19}{c}{SYNTHIA -\textgreater CityScpaes}  \\ \hline
% \multicolumn{1}{l|}{OSBP (ECCV 2018)}       &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{UAN (CVPR 2021)}        &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{UniOT (NeuIPS 2022)}    &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \multicolumn{1}{l|}{AdapSegNet (CVPR 2018)} &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{Pixmatch (CVPR2021)}    &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{DAFormer (CVPR 2022)}   &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{HRDA (ECCV 2022)}       &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\
% \multicolumn{1}{l|}{MIC (CVPR 2023)}        &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \multicolumn{1}{l|}{\textbf{Ours}}          &                          &                            &                            &                          &                           &      &                           &                            &                         &                            &       &                         &                         &                            & \multicolumn{1}{l|}{}     &                            &                             &                             \\ \hline
% \end{tabular}
% }
% \end{table*}


==> sec_final/table/suppl_main.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{2.pt}
\renewcommand{\arraystretch}{1.2}

\begin{NiceTabular}{l|ccccccccccccc|ccc}
\specialrule{1.5pt}{1pt}{0pt}
\multicolumn{1}{l|}{Method}                                & Road  & S.walk & Build. & Wall  & Fence & Light & Veget. & Terrain & Sky   & Car   & Bus   & M.bike & \multicolumn{1}{c|}{Bike}  & Common & Private & H-Score \\ \hline
\multicolumn{17}{c}{\textbf{GTA5 $\rightarrow$ Cityscapes}}                                                                                                                                                                 \\ \hline
\multicolumn{1}{l}{DAF~\cite{hoyer2022daformer}}         & 95.80 & 65.37  & 87.12  & 54.08 & 45.81 & 51.78 & 89.20  & 42.93   & 91.03 & 89.19 & 37.93 & 50.54  & \multicolumn{1}{c}{48.49} & 66.09  & 29.23   & 40.53   \\
\rowcolor[gray]{.9}\multicolumn{1}{l}{DAF + BUS}   & 91.90 & 41.06  & 88.04  & 48.65 & 48.74 & 48.94 & 89.59  & 44.37   & 91.61 & 89.99 & 46.09  & 48.49   & \multicolumn{1}{c}{62.47}  &  64.61 & 39.23    & 48.82     \\
\multicolumn{1}{l}{HRDA~\cite{hoyer2022hrda}}             & 95.31 & 37.70  & 89.26  & 57.41 & 37.00 & 61.16 & 90.96  & 46.86   & 94.39 & 93.39 & 62.45 & 58.13  & \multicolumn{1}{c}{65.71} &  68.44 & 31.02   & 42.70   \\
\rowcolor[gray]{.9}\multicolumn{1}{l}{HRDA + BUS}       & 88.07 & 39.59  & 88.57  & 55.12 & 48.29 & 56.24 & 90.02  & 46.30   & 91.76 & 92.03 & 46.96 & 57.10  & \multicolumn{1}{c}{66.02} &  66.62 & 42.50   & 51.89   \\
\multicolumn{1}{l}{MIC~\cite{hoyer2023mic}}              & 97.14 & 79.45   & 88.78  & 55.6  & 53.92  & 26.11 & 89.94  & 50.98   & 93.54 & 92.46 & 69.09 & 54.53  & \multicolumn{1}{c}{63.43}  & 70.38  & 31.78    & 43.79   \\
\rowcolor[gray]{.9}\multicolumn{1}{l}{MIC + BUS (Ours)} & 95.19 & 66.36  & 90.36  & 57.20 & 56.17 & 56.68 & 91.07  & 49.46   & 93.29 & 93.55 & 64.79 & 58.03  & \multicolumn{1}{c}{68.21} &  72.33  &  53.95   &  61.81   \\
\specialrule{1.5pt}{1pt}{1pt}
\end{NiceTabular}%
}
\vspace{-2mm}
\caption{\label{tab:others} Comparison result of some self-training based UDA methods with head-expansion and applying BUS respectively on GTA5 $\rightarrow$ Cityscapes. DAF denotes DAFormer~\cite{hoyer2022daformer}.}
\end{table*}

==> sec_final/table/table.tex <==


\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{Cityscapes $\rightarrow$ IDD} & \multicolumn{3}{c}{Cityscapes $\rightarrow$ SYNTHIA} \\ \cline{2-7} 
                        & Common      & Private      & H-Score     & Common    & Private    & H-Score    \\ \hline
BUDA                    & 37.3        & 18.5         & 24.7         & 36.2        & 17.0         & 23.1        \\
MIC                     &   54.3        &    24.1      &    34.4       & 61.80        & 1.8       & 3.5       \\
\textbf{BUS}            & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}         & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}        \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
%\caption{\label{tab:BUDA_experiment} Comparison of BUS with BUDA on private classes 'auto rickshaw' and 'animal'.}
\caption{\label{tab:BUDA_experiment} Additional experiments on CS $\rightarrow$ IDD.}%Comparison of BUS with BUDA.}
\vspace{-4mm}
\end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
Method & Common & Private & H-Score \\ \hline
MIC    & 60.35 \(\pm\) 6.55 & 61.38 \(\pm\) 10.61   & 59.66 \(\pm\) 11.13   \\
\textbf{BUS}    & \textbf{64.16 \(\pm\) 7.07}  & \textbf{66.22 \(\pm\) 11.77}   & \textbf{64.33 \(\pm\) 3.45}   \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
\caption{\label{tab:random_private} H-Score on randomly selecting unseen classes.}
\vspace{-3mm}
\end{table}

\begin{table}[t]
\centering
\setlength{\tabcolsep}{10.5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\specialrule{1.0pt}{0.1pt}{0pt}
\hline
\multirow{2}{*}{Method} & \multicolumn{3}{c|}{SYNTHIA $\rightarrow$ Cityscapes} & \multicolumn{3}{c}{Cityscapes $\rightarrow$ IDD} \\ \cline{2-7} 
                        & Common      & Private      & H-Score     & Common    & Private    & H-Score    \\ \hline
BUDA                    & 36.2        & 17.0         & 23.1         & 37.3        & 18.5       & 24.7        \\
MIC                     & 61.80          & 1.8         & 3.5         & 54.3        & 24.1       & 34.4        \\
\textbf{BUS}                    & 0.0          & 0.0         & 0.0         & \textbf{55.6}        & \textbf{39.7}       & \textbf{46.3}        \\ \hline
\specialrule{1.0pt}{0.2pt}{1pt}
\end{tabular}%
}
\vspace{-4mm}
%\caption{\label{tab:BUDA_experiment} Comparison of BUS with BUDA on private classes 'auto rickshaw' and 'animal'.}
\caption{\label{tab:BUDA_experiment} Additional experiments on CS $\rightarrow$ IDD.}%Comparison of BUS with BUDA.}
\vspace{-4mm}
\end{table}
